Data Optimisation of Machine Learning Models for Smart Irrigation in Urban Parks

Urban environments face significant challenges due to climate change, including extreme heat, drought, and water scarcity, which impact public health, community well-being, and local economies. Effective management of these issues is crucial, particularly in areas like Sydney Olympic Park, which relies on one of Australia's largest irrigation systems. The Smart Irrigation Management for Parks and Cool Towns (SIMPaCT) project, initiated in 2021, leverages advanced technologies and machine learning models to optimize irrigation and induce physical cooling. This paper introduces two novel methods to enhance the efficiency of the SIMPaCT system's extensive sensor network and applied machine learning models. The first method employs clustering of sensor time series data using K-shape and K-means algorithms to estimate readings from missing sensors, ensuring continuous and reliable data. This approach can detect anomalies, correct data sources, and identify and remove redundant sensors to reduce maintenance costs. The second method involves sequential data collection from different sensor locations using robotic systems, significantly reducing the need for high numbers of stationary sensors. Together, these methods aim to maintain accurate soil moisture predictions while optimizing sensor deployment and reducing maintenance costs, thereby enhancing the efficiency and effectiveness of the smart irrigation system. Our evaluations demonstrate significant improvements in the efficiency and cost-effectiveness of soil moisture monitoring networks. The cluster-based replacement of missing sensors provides up to 5.4% decrease in average error. The sequential sensor data collection as a robotic emulation shows 17.2% and 2.1% decrease in average error for circular and linear paths respectively.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> cut_text.tex <==
\section{Related work - old}
This paper ...
\todo[inline]{\textit{Nasser}\\Write and organize the related work}

Smart sensors commonly ... \cite{soussi2024sur}
Time series clustering using k-shape and DTW has been widely studied for various applications, including hydrological data analysis. Paparrizos and Gravano proposed the k-shape algorithm, which outperforms traditional k-means and DTW approaches for time series clustering.  \cite{prakaisak2022hydrological}.
Sardá-Espinosa compared the performance of different time series clustering algorithms, including k-shape and DTW, using the dtwclust package in R \cite{sarda2017comparing}.
\\
Handling missing data or disconnected sensors is a crucial aspect when working with sensor networks. Imputation techniques are often employed to estimate missing values based on available data from other sensors in the same cluster. Nourani et al. used robust clustering methods to assess the spatiotemporal variability of groundwater quantity and quality, including handling missing data. \cite{lee2020clustering}.
Moazamnia et al. formulated a genetic algorithm-based self-organizing map (GA-SOM) for managing aquifer heterogeneity and predicting groundwater levels, which can handle missing data. \cite{azmat2022forecasting}.`


In \cite{guyeux2019introducing}
  Introducing and comparing recent clustering methods for massive data management in the internet of things,
  
In \cite{alkawsi2023towards}
  Towards lowering computational power in IoT systems: Clustering algorithm for high-dimensional data stream using entropy window reduction
  

In \cite{alam2020error}
  Error-aware data clustering for in-network data reduction in wireless sensor networks

In \cite{zhang2023autonomous}
  Autonomous Internet of Things (IoT) Data Reduction Based on Adaptive Threshold
  

In \cite{ramesh2024transfer}
  Transfer learning approach to reduce similar IOT sensor data for industrial applications\\

in \cite{gong2023spatiotemporally} revealed that reducing precision has a positive effect on reducing I/O and storage for sensors.\\
in \cite{de2022aiquam} uses categorized indexes for ...
\\
Other applications in environmental and related domains:
Clustering for climate \cite{mohanty2023detection}

DTW Clustering for oil prediction \cite{prasetyo2021clustering}.

Clustering for outlier detection in river water quality in \cite{lu2024design}.

Clustering time series for road co2 emissions in \cite{de2023time}.

Clustering for intake water to industrial parks in \cite{chen2024using}.


\\ auto methods\\
\subsubsection{Auto DTW-based k-means}
Auto DTW-based K-means is our proposed extension of the k-means clustering algorithm with DTW that aims to find the optimal number of clusters by evaluating the quality of clustering for different values of $k$ within a specified range $[k_{min}, k_{max}]$. The optimal $k$ is determined based on a clustering quality metric, the silhouette score. \\

\textbf{Auto DTW-based K-means Algorithm:}
The Auto DTW-based K-means algorithm follows these steps:

Initialize $k_{min}$ and $k_{max}$ to define the range of $k$ values to explore.
For each $k$ in the range $[k_{min}, k_{max}]$:

Perform k-means clustering with DTW using the current value of $k$.
Compute the silhouette score for the resulting clustering.


Select the optimal $k$ that maximizes the silhouette score:



\begin{equation}
k_{opt} = \argmax_{k \in [k_{min}, k_{max}]} silhouette(k)
\end{equation}

Return the clustering result obtained with $k_{opt}$ as the optimal clustering.
Time Complexity:
The time complexity of Auto DTW-based K-means is $O((k_{max} - k_{min} + 1) \cdot T \cdot N^2 \cdot m^2)$, where $T$ is the number of iterations for each k-means clustering run, $N$ is the number of time series, and $m$ is the average length of the time series. The DTW distance computation has a time complexity of $O(m^2)$ for each pair of time series, and the silhouette score computation has a time complexity of $O(N^2)$ for each clustering result.

\subsubsection{Auto K-shape}
Auto K-shape is our proposed extension of the k-shape clustering algorithm that aims to find the optimal number of clusters by evaluating the quality of clustering for different values of $k$ within a specified range $[k_{min}, k_{max}]$. The optimal $k$ is determined based on a clustering quality metric, the silhouette score. \\
\textbf{Auto K-shape Algorithm:}
The Auto K-shape algorithm follows these steps:

Initialize $k_{min}$ and $k_{max}$ to define the range of $k$ values to explore.
For each $k$ in the range $[k_{min}, k_{max}]$:

Perform k-shape clustering with the current value of $k$.
Compute the silhouette score for the resulting clustering.


Select the optimal $k$ that maximizes the silhouette score:



\begin{equation}
k_{opt} = \argmax_{k \in [k_{min}, k_{max}]} silhouette(k)
\end{equation}

Return the clustering result obtained with $k_{opt}$ as the optimal clustering.
Time Complexity:
The time complexity of Auto K-shape is $O((k_{max} - k_{min} + 1) \cdot T \cdot N^2)$, where $T$ is the number of iterations for each k-shape clustering run, and $N$ is the number of time series. The silhouette score computation has a time complexity of $O(N^2)$ for each clustering result.


\\t comp\\
Time Complexity:
The time complexity of k-means clustering with DTW is $O(TKNm^2)$, where $T$ is the number of iterations, $K$ is the number of clusters, $N$ is the number of time series, and $m$ is the average length of the time series. The DTW distance computation has a time complexity of $O(m^2)$ for each pair of time series.


